Understanding the Tradeoffs in Client-side Privacy for Downstream Speech Tasks

As users increasingly rely on cloud-based computing services, it is important to ensure that uploaded speech data remains private. Existing solutions rely either on server-side methods or focus on hiding speaker identity. While these approaches reduce certain security concerns, they do not give users client-side control over whether their biometric information is sent to the server. In this paper, we formally define client-side privacy and discuss its three unique technical challenges: (1) direct manipulation of raw data on client devices, (2) adaptability with a broad range of server-side processing models, and (3) low time and space complexity for compatibility with limited-bandwidth devices. Solving these challenges requires new models that achieve high-fidelity reconstruction, privacy preservation of sensitive personal attributes, and efficiency during training and inference. As a step towards client-side privacy for speech recognition, we investigate three techniques spanning signal processing, disentangled representation learning, and adversarial training. Through a series of gender and accent masking tasks, we observe that each method has its unique strengths, but none manage to effectively balance the trade-offs between performance, privacy, and complexity. These insights call for more research in client-side privacy to ensure a safer deployment of cloud-based speech processing services.

==> PaperSample_Guideline_tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{chen2020fedhealth}
Y.~Chen \emph{et~al.}, ``Fedhealth: A federated transfer learning framework for
  wearable healthcare,'' \emph{IEEE Intelligent Systems}, 2020.

\bibitem{geyer2017differentially}
R.~C. Geyer, T.~Klein, and M.~Nabi, ``Differentially private federated
  learning: A client level perspective,'' \emph{arXiv preprint
  arXiv:1712.07557}, 2017.

\bibitem{liang2020think}
P.~P. Liang \emph{et~al.}, ``Think locally, act globally: Federated learning
  with local and global representations,'' \emph{arXiv preprint
  arXiv:2001.01523}, 2020.

\bibitem{xu2019federated}
J.~Xu and F.~Wang, ``Federated learning for healthcare informatics,''
  \emph{Journal of Healthcare Informatics Research}, pp. 1 -- 19, 2021.

\bibitem{mcgraw2016personalized}
I.~McGraw \emph{et~al.}, ``Personalized speech recognition on mobile devices,''
  \emph{ICASSP}, pp. 5955--5959, 2016.

\bibitem{gong2020cloud}
X.~Gong \emph{et~al.}, ``Model extraction attacks and defenses on cloud-based
  machine learning models,'' \emph{IEEE Communications Magazine}, vol.~58,
  no.~12, pp. 83--89, 2020.

\bibitem{anggraini2018speech}
N.~Anggraini, A.~Kurniawan, L.~K. Wardhani, and N.~Hakiem, ``Speech recognition
  application for the speech impaired using the android-based google cloud
  speech api,'' \emph{Telkomnika}, vol.~16, no.~6, pp. 2733--2739, 2018.

\bibitem{leroy2019federated}
D.~Leroy \emph{et~al.}, ``Federated learning for keyword spotting,''
  \emph{ICASSP}, pp. 6341--6345, 2019.

\bibitem{singh2019profiling}
R.~Singh, \emph{Profiling Humans from their Voice}.\hskip 1em plus 0.5em minus
  0.4em\relax Springer Singapore, 2019.

\bibitem{jing1999client}
J.~Jing, A.~S. Helal, and A.~Elmagarmid, ``Client-server computing in mobile
  environments,'' \emph{CSUR}, vol.~31, no.~2, pp. 117--157, 1999.

\bibitem{li2020federated}
T.~Li, A.~K. Sahu, A.~Talwalkar, and V.~Smith, ``Federated learning:
  Challenges, methods, and future directions,'' \emph{IEEE Signal Processing
  Magazine}, vol.~37, no.~3, pp. 50--60, 2020.

\bibitem{caldas2018leaf}
S.~Caldas \emph{et~al.}, ``Leaf: A benchmark for federated settings,''
  \emph{Workshop on Federated Learning for Data Privacy and Confidentiality},
  2018.

\bibitem{hwang2011serverclient}
J.-J. Hwang, H.-K. Chuang, Y.-C. Hsu, and C.-H. Wu, ``A business model for
  cloud computing based on a separate encryption and decryption service,'' in
  \emph{2011 International Conference on Information Science and Applications},
  2011, pp. 1--7.

\bibitem{zhao2019secure}
C.~Zhao \emph{et~al.}, ``Secure multi-party computation: Theory, practice and
  applications,'' \emph{IS}, vol. 476, pp. 357--372, 2019.

\bibitem{sun2018private}
X.~Sun \emph{et~al.}, ``Private machine learning classification based on fully
  homomorphic encryption,'' \emph{IEEE Transactions on Emerging Topics in
  Computing}, vol.~8, no.~2, pp. 352--364, 2018.

\bibitem{papernot2018scalable}
N.~Papernot \emph{et~al.}, ``Scalable private learning with {PATE},''
  \emph{ICLR}, 2018.

\bibitem{abadi2016deep}
M.~Abadi \emph{et~al.}, ``Deep learning with differential privacy,'' in
  \emph{Proceedings of the 2016 ACM SIGSAC conference on computer and
  communications security}, 2016, pp. 308--318.

\bibitem{de2020overview}
E.~De~Cristofaro, ``A critical overview of privacy in machine learning,''
  \emph{IEEE Security Privacy}, vol.~19, no.~4, pp. 19--27, 2021.

\bibitem{wilson2014share}
D.~C. Wilson and G.~Ateniese, ``“to share or not to share” in client-side
  encrypted clouds,'' in \emph{ICIS}.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2014, pp. 401--412.

\bibitem{silessi2016lexical}
S.~Silessi, C.~Varol, and M.~Karabatak, ``Identifying gender from sms text
  messages,'' in \emph{ICMLA}, 2016, pp. 488--491.

\bibitem{reza2017sensitive}
R.~Shokri, M.~Stronati, C.~Song, and V.~Shmatikov, ``Membership inference
  attacks against machine learning models,'' in \emph{2017 IEEE Symposium on
  Security and Privacy (SP)}, 2017, pp. 3--18.

\bibitem{caliskan2014privacy}
A.~Caliskan~Islam, J.~Walsh, and R.~Greenstadt, ``Privacy detective: Detecting
  private information and collective privacy behavior in a large social
  network,'' in \emph{Proceedings of the 13th Workshop on Privacy in the
  Electronic Society}, 2014, pp. 35--46.

\bibitem{sun2019mitigating}
T.~Sun \emph{et~al.}, ``Mitigating gender bias in natural language processing:
  Literature review,'' in \emph{ACL}, 2019.

\bibitem{baevski2020wav2vec}
A.~Baevski, H.~Zhou, A.~Mohamed, and M.~Auli, ``wav2vec 2.0: A framework for
  self-supervised learning of speech representations,'' \emph{NeurIPS}, 2020.

\bibitem{kak1977speech}
S.~C. Kak and N.~Jayant, ``On speech encryption using waveform scrambling,''
  \emph{Bell System Technical Journal}, vol.~56, no.~5, pp. 781--808, 1977.

\bibitem{sridharan1991fast}
S.~Sridharan, E.~Dawson, and B.~Goldburg, ``Fast fourier transform based speech
  encryption system,'' \emph{IEE Proceedings I-Communications, Speech and
  Vision}, vol. 138, no.~3, pp. 215--223, 1991.

\bibitem{smaragdis2007smc_asr}
P.~Smaragdis and M.~Shashanka, ``A framework for secure speech recognition,''
  \emph{TASLP}, vol.~15, no.~4, pp. 1404--1413, 2007.

\bibitem{jin2009speaker}
Q.~Jin, A.~R. Toth, T.~Schultz, and A.~W. Black, ``Speaker de-identification
  via voice transformation,'' in \emph{ASRU}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2009, pp. 529--533.

\bibitem{tomashenko2020introducing}
N.~Tomashenko \emph{et~al.}, ``Introducing the voiceprivacy initiative,''
  \emph{Interspeech}, 2020.

\bibitem{aloufi2020privacy}
R.~Aloufi, H.~Haddadi, and D.~Boyle, ``Privacy-preserving voice analysis via
  disentangled representations,'' \emph{ACM SIGSAC}, 2020.

\bibitem{ahmed_preech_privacy_server}
S.~Ahmed, A.~R. Chowdhury, K.~Fawaz, and P.~Ramanathan, ``Preech: A system for
  privacy-preserving speech transcription,'' in \emph{USENIX}.\hskip 1em plus
  0.5em minus 0.4em\relax {USENIX} Association, Aug. 2020, pp. 2703--2720.

\bibitem{ma_fei_privacy_server}
Z.~{Ma}, Y.~{Liu}, X.~{Liu}, J.~{Ma}, and F.~{Li}, ``Privacy-preserving
  outsourced speech recognition for smart iot devices,'' \emph{IEEE Internet of
  Things Journal}, vol.~6, no.~5, pp. 8406--8420, 2019.

\bibitem{nautsh2019speaker}
A.~Nautsch \emph{et~al.}, ``Preserving privacy in speaker and speech
  characterisation,'' \emph{CSL}, vol.~58, pp. 441--480, 2019.

\bibitem{srivastava2020design_vc}
B.~M.~L. Srivastava \emph{et~al.}, ``Design choices for x-vector based speaker
  anonymization,'' \emph{Interspeech}, 2020.

\bibitem{huang2020sequence_vc_shinji}
W.-C. Huang, T.~Hayashi, S.~Watanabe, and T.~Toda, ``The sequence-to-sequence
  baseline for the voice conversion challenge 2020: Cascading asr and tts,''
  \emph{arXiv preprint arXiv:2010.02434}, 2020.

\bibitem{sisman2021vc}
B.~Sisman, J.~Yamagishi, S.~King, and H.~Li, ``An overview of voice conversion
  and its challenges: From statistical modeling to deep learning,''
  \emph{TASLP}, vol.~29, pp. 132--157, 2021.

\bibitem{zheng2020automatic}
L.~Zheng \emph{et~al.}, ``When automatic voice disguise meets automatic speaker
  verification,'' \emph{IEEE Transactions on Information Forensics and
  Security}, vol.~16, pp. 824--837, 2020.

\bibitem{noe2020adversarial}
P.-G. No{\'e} \emph{et~al.}, ``Adversarial disentanglement of speaker
  representation for attribute-driven privacy preservation,'' \emph{arXiv
  preprint arXiv:2012.04454}, 2020.

\bibitem{ericsson2020adversarial_amnist}
D.~Ericsson \emph{et~al.}, ``Adversarial representation learning for private
  speech generation,'' \emph{arXiv preprint arXiv:2006.09114}, 2020.

\bibitem{chen2007using}
J.~Chen \emph{et~al.}, ``Using keyword spotting and replacement for speech
  anonymization,'' in \emph{ICME}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2007, pp. 548--551.

\bibitem{kondo2014genderbabble}
K.~Kondo and H.~Sakurai, ``Gender-dependent babble maskers created from
  multi-speaker speech for speech privacy protection,'' in \emph{2014 Tenth
  International Conference on Intelligent Information Hiding and Multimedia
  Signal Processing}, 2014, pp. 251--254.

\bibitem{stoidis2021protecting}
D.~Stoidis and A.~Cavallaro, ``Protecting gender and identity with disentangled
  speech representations,'' \emph{arXiv preprint arXiv:2104.11051}, 2021.

\bibitem{panayotov2015librispeech}
V.~Panayotov, G.~Chen, D.~Povey, and S.~Khudanpur, ``Librispeech: an asr corpus
  based on public domain audio books,'' in \emph{ICASSP}.\hskip 1em plus 0.5em
  minus 0.4em\relax IEEE, 2015, pp. 5206--5210.

\bibitem{ji2014differential}
Z.~Ji, Z.~C. Lipton, and C.~Elkan, ``Differential privacy and machine learning:
  a survey and review,'' \emph{arXiv preprint arXiv:1412.7584}, 2014.

\bibitem{wu2019ordinal}
P.~Wu, S.~K. Rallabandi, A.~W. Black, and E.~Nyberg, ``Ordinal triplet loss:
  Investigating sleepiness detection from speech.'' in \emph{Interspeech},
  2019, pp. 2403--2407.

\bibitem{wu2020automatically}
P.~Wu, Y.~Zhong, and A.~W. Black, ``Automatically identifying language family
  from acoustic examples in low resource scenarios,'' \emph{arXiv preprint
  arXiv:2012.00876}, 2020.

\bibitem{liang2020cross}
P.~P. Liang, P.~Wu, L.~Ziyin, L.-P. Morency, and R.~Salakhutdinov,
  ``Cross-modal generalization: Learning in low resource modalities via
  meta-alignment,'' \emph{arXiv preprint arXiv:2012.02813}, 2020.

\bibitem{wang2017gender}
Y.~Wang, J.~Du, L.-R. Dai, and C.-H. Lee, ``A gender mixture detection approach
  to unsupervised single-channel speech separation based on deep neural
  networks,'' \emph{TASLP}, vol.~25, no.~7, pp. 1535--1546, 2017.

\bibitem{mousa2010voice}
A.~Mousa, ``Voice conversion using pitch shifting algorithm by time stretching
  with psola and re-sampling,'' \emph{Journal of electrical engineering},
  vol.~61, no.~1, p.~57, 2010.

\bibitem{laskar2012pitch}
R.~H. Laskar, K.~Banerjee, F.~A. Talukdar, and K.~S. Rao, ``A pitch synchronous
  approach to design voice conversion system using source-filter correlation,''
  \emph{International Journal of Speech Technology}, vol.~15, no.~3, pp.
  419--431, 2012.

\bibitem{disentangle_vae_avc}
J.-c. Chou and H.-y. Lee, ``One-shot voice conversion by separating speaker and
  content representations with instance normalization,'' in \emph{Interspeech},
  2019.

\bibitem{burgess2018understanding}
C.~P. Burgess \emph{et~al.}, ``Understanding disentangling in $\beta$-vae,''
  \emph{arXiv preprint arXiv:1804.03599}, 2018.

\bibitem{griffin_lim}
D.~{Griffin} and {Jae Lim}, ``Signal estimation from modified short-time
  fourier transform,'' \emph{IEEE Transactions on Acoustics, Speech, and Signal
  Processing}, vol.~32, no.~2, pp. 236--243, 1984.

\bibitem{ulyanov2016instance}
D.~Ulyanov, A.~Vedaldi, and V.~Lempitsky, ``Instance normalization: The missing
  ingredient for fast stylization,'' \emph{arXiv preprint arXiv:1607.08022},
  2016.

\bibitem{huang_adaIN}
X.~{Huang} and S.~{Belongie}, ``Arbitrary style transfer in real-time with
  adaptive instance normalization,'' in \emph{ICCV}, 2017, pp. 1510--1519.

\bibitem{yoo2020cyclevaegan}
I.-C. Yoo \emph{et~al.}, ``Speaker anonymization for personal information
  protection using voice conversion techniques,'' \emph{IEEE Access}, vol.~8,
  pp. 198\,637--198\,645, 2020.

\bibitem{dhariwal2020jukebox}
P.~Dhariwal \emph{et~al.}, ``Jukebox: A generative model for music,''
  \emph{arXiv preprint arXiv:2005.00341}, 2020.

\bibitem{rallabandi2019submission}
S.~Rallabandi, P.~Wu, and A.~W. Black, ``Submission from cmu for blizzard
  challenge 2019,'' \emph{Proceedings of Blizzard Challenge}, vol. 2019, 2019.

\bibitem{ranzato2014video}
M.~Ranzato \emph{et~al.}, ``Video (language) modeling: a baseline for
  generative models of natural videos,'' \emph{arXiv preprint arXiv:1412.6604},
  2014.

\bibitem{chou_gan}
J.-c. Chou, C.-c. Yeh, H.-y. Lee, and L.-S. Lee, ``Multi-target voice
  conversion without parallel data by adversarially learning disentangled audio
  representations,'' in \emph{Interspeech}, 2018.

\bibitem{zhou2021gan}
K.~Zhou, B.~Sisman, R.~Liu, and H.~Li, ``Seen and unseen emotional style
  transfer for voice conversion with a new emotional speech dataset,'' in
  \emph{ICASSP}, 2021, pp. 920--924.

\bibitem{goodfellow2014generative}
I.~Goodfellow \emph{et~al.}, ``Generative adversarial nets,'' \emph{NIPS},
  vol.~27, 2014.

\bibitem{oord2016wavenet}
A.~v.~d. Oord \emph{et~al.}, ``Wavenet: A generative model for raw audio,'' in
  \emph{SSW}, 2016.

\bibitem{veaux2016vctk}
C.~Veaux, J.~Yamagishi, K.~MacDonald \emph{et~al.}, ``{CSTR} {VCTK} corpus:
  English multi-speaker corpus for cstr voice cloning toolkit,''
  \emph{University of Edinburgh}, 2017.

\bibitem{voxceleb_vggvox}
A.~Nagrani, J.~S. Chung, and A.~Zisserman, ``Voxceleb: A large-scale speaker
  identification dataset,'' in \emph{Interspeech}, 2017.

\bibitem{simonyan2014vgg}
K.~Simonyan and A.~Zisserman, ``Very deep convolutional networks for
  large-scale image recognition,'' in \emph{ICLR}, 2015.

\bibitem{watanabe2018espnet}
S.~Watanabe \emph{et~al.}, ``{ESPnet}: End-to-end speech processing toolkit,''
  in \emph{Interspeech}, 2018, pp. 2207--2211.

\bibitem{goodfellow2014explaining}
I.~Goodfellow, J.~Shlens, and C.~Szegedy, ``Explaining and harnessing
  adversarial examples,'' in \emph{ICLR}, 2015.

\bibitem{higgins2016beta}
I.~Higgins, L.~Matthey, A.~Pal, C.~Burgess, X.~Glorot, M.~Botvinick,
  S.~Mohamed, and A.~Lerchner, ``beta-vae: Learning basic visual concepts with
  a constrained variational framework,'' \emph{ICLR}, 2016.

\bibitem{locatello2019challenging}
F.~Locatello, S.~Bauer, M.~Lucic, G.~Raetsch, S.~Gelly, B.~Sch{\"o}lkopf, and
  O.~Bachem, ``Challenging common assumptions in the unsupervised learning of
  disentangled representations,'' in \emph{ICML}.\hskip 1em plus 0.5em minus
  0.4em\relax PMLR, 2019, pp. 4114--4124.

\end{thebibliography}

